CheckDP: An Automated and Integrated Approach for Proving Differential Privacy or Finding Precise Counterexamples

We propose CheckDP, the first automated and integrated approach for proving or disproving claims that a mechanism is differentially private. CheckDP can find counterexamples for mechanisms with subtle bugs for which prior counterexample generators have failed. Furthermore, it was able to \emph{automatically} generate proofs for correct mechanisms for which no formal verification was reported before. CheckDP is built on static program analysis, allowing it to be more efficient and more precise in catching infrequent events than existing counterexample generators (which run mechanisms hundreds of thousands of times to estimate their output distribution). Moreover, its sound approach also allows automatic verification of correct mechanisms. When evaluated on standard benchmarks and newer privacy mechanisms, CheckDP generates proofs (for correct mechanisms) and counterexamples (for incorrect mechanisms) within 70 seconds without any false positives or false negatives.

==> fig_semantics.tex <==
\begin{figure}[ht]
\small 
\vspace{-0.6cm}
\begin{align*}
\trans{\skipcmd}_\store &= \unitop~m \\
\trans{x:=e}_\store &= \unitop~(\subst{m}{x}{\evalexpr{e}{m}}) \\
\trans{\eta:=g}_\store &= \bindop~\evalexpr{g}{}~(\lambda v.~\unitop~\subst{m}{\eta }{v}) \\
\trans{c_1;c_2}_\store &= \bindop~(\evalexpr{c_1}{\store})~\trans{c_2}  \\
\trans{\ifcmd{e}{c_1}{c_2}}_\store &= 
        \begin{cases} 
        \trans{c_1}_\store &\mbox{if } \evalexpr{e}{\store} = \true \\
        \trans{c_2}_\store &\mbox{if } \evalexpr{e}{\store} = \false \\
        \end{cases} \\
\trans{\whilecmd{e}{c}}_\store &= w^*~m\\
\text{where } w^*              &= fix (\lambda f.~\lambda m. \code{if}~\evalexpr{e}{m}=\true\\
                                \code{then}~&(\bindop~\evalexpr{c}{m}~f)~\code{else}~{(\unitop~m)}) \\
\trans{c;\outcmd{e}}_\store &= \bindop~(\evalexpr{c}{\store})~(\lambda m'.~\unitop~\evalexpr{e}{m'})
\end{align*}
\caption{\tool: language semantics.}
\label{fig:semantics}
\end{figure}


==> fig_template_rules.tex <==
\begin{figure*}
\raggedright
\setstretch{0.85}
\begin{mathpar}
\inferrule*[right=(T-Assert)]
{T = \code{GenerateTemplate}(G, \lambda, L[\lambda])}
{\proves \flowrule{\Gamma}{\eta := \lapm{r}~\real}{\vpriv{\priv} := \vpriv{\priv}+|T|/r;\distance{$\eta$} := T;}{\Gamma'}}
\and
\inferrule*[right=(T-Laplace)]
{ }
{\proves \flowrule{\Gamma}{}{\vpriv{\priv} := \vpriv{\priv}+|T|/r;\distance{$\eta$} := T;}{\Gamma'}}
\end{mathpar}
\caption{Rules for generating the alignment templates.\label{fig:template_rules}}
\end{figure*}

==> sec_limitations.tex <==

\tool relies on the underlying randomness alignment proving technique; hence is subject to its limitations, including lack of support for $(\epsilon, \delta)$-differential privacy and renyi differential privacy~\cite{M2017:Renyi}. Moreover, subtle mechanisms such as PrivTree~\cite{privtree} and private selection~\cite{privateselection}, where the costs of intermediate results are dependent on the data but the cost of sum is data-independent, is still out of reach for randomness alignment (hence \tool). 

\move{\paragraph*{Expressiveness of Alignment}
Recently, Noisy Max with Gap (and a more general version Noisy Top-K with Gap)~\cite{freegap} is proposed with a manual randomness alignment proof. This mechanism improves existing Noisy Max and releases the gap between the max and the runner-up for free. To prove this mechanism using randomness alignment,  the gap between the current maximum query answer and runner-up needs to be aligned between two related executions to produce the same result. This requires \tool to keep the alignments of the current maximum \emph{and} the runner-up, and erase all other ones (a key in proving Noisy Max-like mechanisms). However, the current form of \tool, though equipped with shadow execution, lacks the expressiveness to keep or erase arbitrary number of alignments.}

\tool is designed for DP mechanisms, rather than larger programs built on top of them. An interesting area of future work is integrating \tool with tools like DFuzz~\cite{DFuzz}, which are more efficient on programs built on top of DP mechanisms (but don't verify the mechanisms themselves).






==> tab_comparison.tex <==
\begin{table*}
\centering
\small{
\caption{Comparisons. $\#t$ stands for $\true$ and $\#f$ stands for $\false$.\label{tab:counterexamples}}
\small
\begin{tabular}{ccccccccc}
\Xhline{1.5\arrayrulewidth}
\multicolumn{1}{c}{\textbf{Mechanism}} & \code{q} & \code{q}$'$ & \multicolumn{1}{c}{\code{size}} & \multicolumn{1}{c}{\textbf{Extra Args}}& \multicolumn{1}{c}{\textbf{Output}} & \multicolumn{1}{c}{\textbf{Iterations}} & \multicolumn{1}{c}{\textbf{Time(s)}} \\
\Xhline{1\arrayrulewidth}
BadNoisyMax & $[0, 0, 0, 0, 0]$ & $[-1, 1, 1, 1, 1]$ & 5 & N/A & $0$ & 3 &  5.74  \\
BadGapSVT & $[0, 0, 0, 0, 0]$ & $[1, 1, 1, 1, -1]$ & 5 & $T$: 0, $N$: 1 & \makecell{$[0, 0, 0, 0,1]$} & 4 &  5.77 \\
BadSVT1 & $[0, 0, 0, 0, 1]$ & $[1, 1, 1, 1, 0]$ & 5 & $T$: 0, $N$: 1 & \makecell{$[\#f, \#f, \#f, \#f, \#t]$} & 4 & 3.23 \\
BadSVT2 & $[0, 0, 0, 0, 0]$ & $[1, 1, 1, 1, -1]$ & 5 & $T$: 0, $N$: 1 & \makecell{$[\#f, \#f, \#f, \#f, \#t]$} & 4 & 4.79  \\
BadSVT3         & $[0, 0, 0, 0, 0]$ & $[1, 1, 1, 1, -1]$ & 5 & $T$: 0, $N$: 1 &\makecell{$[\#f, \#f, \#f, \#f, \#t]$} & 4 & 5.27     \\ 
BadSmartSum & $[0, 0, 0, 0, 0]$ & $[0, 0, 0, 1, 0]$ & 5 & $T$: 4, $M$: 4  & \makecell{$[0,0,0,0,0]$} & 4 & 6.32 \\
BadPartialSum & $[0, 0, 0, 0, 0]$ & $[0, 0, 0, 0, 1]$ & 5 & N/A & \makecell{$0$} & 3 & 3.71\\
\Xhline{1.5\arrayrulewidth} 
\end{tabular}}
\end{table*}

